Taming Timeout Flakiness: An Empirical Study of SAP HANA

Regression testing aims to prevent code changes from breaking existing features. Flaky tests negatively affect regression testing because they result in test failures that are not necessarily caused by code changes, thus providing an ambiguous signal. Test timeouts are one contributing factor to such flaky test failures. With the goal of reducing test flakiness in SAP HANA, we empirically study the impact of test timeouts on flakiness in system tests. We evaluate different approaches to automatically adjust timeout values, assessing their suitability for reducing execution time costs and improving build turnaround times. We collect metadata on SAP HANA's test executions by repeatedly executing tests on the same code revision over a period of six months. We analyze the test flakiness rate, investigate the evolution of test timeout values, and evaluate different approaches for optimizing timeout values. The test flakiness rate ranges from 49% to 70%, depending on the number of repeated test executions. Test timeouts account for 70% of flaky test failures. Developers typically react to flaky timeouts by manually increasing timeout values or splitting long-running tests. However, manually adjusting timeout values is a tedious task. Our approach for timeout optimization reduces timeout-related flaky failures by 80% and reduces the overall median timeout value by 25%, i.e., blocked tests are identified faster. Test timeouts are a major contributing factor to flakiness in system tests. It is challenging for developers to effectively mitigate this problem manually. Our technique for optimizing timeout values reduces flaky failures while minimizing test costs. Practitioners working on large-scale industrial software systems can use our findings to increase the effectiveness of their system tests while reducing the burden on developers to manually maintain appropriate timeout values.

==> equations/inequality.tex <==
\begin{equation}
\label{eq:cantelli}
    P(X-\overline{X} \geq \lambda Q_n) \leq \frac{1}{n + 1}*\lfloor \frac{n+1}{k^2+1} \rfloor
\end{equation}

==> equations/timeout_cost.tex <==
\begin{equation}
\label{eq:timeout-cost}
    C(x) = \sum_{i=1}^{m} ((1-P(R<x))*\overline{X}_x) + \overline{X}_x \\
    x^* = \underset{x \in \mathbb{N}}{\argmin} \text{ } C(X)
\end{equation}

==> figures/opt_timeout_distribution.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/images/opt_timeout_distribution.pdf}
    \caption{Beanplot that shows the distribution of timeout values after optimization ($n=709$).}
    \label{fig:opt-timeouts-distribution}
\end{figure}

==> sections/70_threats_old.tex <==
\section{Threats to validity}
\label{sec:threats}
In this section, we discuss potential threats to the internal, external, and construct validity of this study. 

\subsection{Internal Validity} 
The internal validity refers to the degree to which we can rule out alternative explanations for our results \cite{brewer2000research}. In the context of this study, the internal validity is mainly threatened by 
Our data collection process is the main threat to the internal validity of our study. Since we calculate the optimal timeouts based on empirical observations on a subset of SAP HANA's tests, our results may be affected by selection bias. To mitigate this threat, we selected tests in consultation with practitioners.

Furthermore, since we test only certain code revisions in our mass testing, our data might be affected by selection bias. For example, one of the revisions could be affected by an actual defect in the code revision under test. To mitigate this threat, we only use revisions that have passed the full pre-submit testing stage of SAP HANA and therefore are unlikely to contain major \chreplaced{defects}{issues}. Furthermore, we did not notice a larger amount of \chreplaced{failures}{errors} during our analysis. \chdeleted{If so, we would have investigated the errors manually.} In summary, we conclude that the impact of defects on our \chreplaced{results}{experiments} is low.

\subsection{External Validity} 
The external validity refers to the degree to which our results generalize to other contexts~\cite{baltes2022sampling}. 

SAP HANA uses a custom testing framework that requires developers to set a timeout value for every test. Therefore, SAP HANA might be particularly affected by test case timeouts. However, previous work targeting large software projects has also identified test case timeout as a common \chadded{flakiness} problem~\cite{parry2021survey, gruber2022survey}. \chadded{Therefore, we assume that our proposed approach to reduce test costs by optimizing timeout values generalizes to software projects suffering from timeout flakiness. } 

\subsection{Construct Validity}
The main threat to the construct validity of our study is \chadded{caused by} the complexity of the SAP HANA test suite. For the purpose of this study, we approximate the cost of a test based on the test execution time. In practice, however, test costs consist of a range of factors, including CPU or RAM usage. Since covering all these factors would be too complex in the SAP HANA testing environment, \chreplaced{researchers and practitioners in the context of SAP HANA}{we} commonly use the execution time as an approximation~\cite{bach2018effects, bach2022testing}.


==> tables/rq1_flakiness.tex <==
\begin{table}
  \begin{center}
  \caption{Flakiness rate across three code revisions based on the MT dataset (\emph{flakiness rate}: number of flaky tests divided by number of unique executed tests; \emph{failure rate}: number of flaky failures divided by number of repeated test executions).}
    \begin{tabular}[width=\textwidth]{l r r r}
    \toprule
       & \textbf{Revision 1} & \textbf{Revision 2} & \textbf{Revision 3} \\
      \midrule
      \textbf{\# Repetitions} & 100 & 120 & 160 \\
      \textbf{Flakiness Rate} & \num{49}\% & \num{64}\% & \num{70}\% \\
      \textbf{\# Unique Tests} & \num{673} & \num{667} & \num{658} \\
      \textbf{\# Flaky Tests} & \num{333} & \num{430} & \num{459} \\
      \textbf{\# 1-20\% failure rate} & 216 & 337 & 342\\
      \textbf{\# 21-40\% failure rate} & 54 & 47 & 54\\
      \textbf{\# 41-60\% failure rate} & 18 & 21 & 27\\
      \textbf{\# 61-80\% failure rate} & 9 & 12 & 10\\
      \textbf{\# 81-99\% failure rate} & 36 & 13 & 26\\
      \bottomrule
      \end{tabular}
    \label{tab:flakiness-across-makes}
  \end{center}
\end{table}
